Reconstructing Materials Tetrahedron: Challenges in Materials Information Extraction

The discovery of new materials has a documented history of propelling human progress for centuries and more. The behaviour of a material is a function of its composition, structure, and properties, which further depend on its processing and testing conditions. Recent developments in deep learning and natural language processing have enabled information extraction at scale from published literature such as peer-reviewed publications, books, and patents. However, this information is spread in multiple formats, such as tables, text, and images, and with little or no uniformity in reporting style giving rise to several machine learning challenges. Here, we discuss, quantify, and document these challenges in automated information extraction (IE) from materials science literature towards the creation of a large materials science knowledge base. Specifically, we focus on IE from text and tables and outline several challenges with examples. We hope the present work inspires researchers to address the challenges in a coherent fashion, providing a fillip to IE towards developing a materials knowledge base.

==> figures/list_of_figures.tex <==
1. Graphical abstract type (lift from outline ppt)
2. Common challenges : 
    4.1.1
    4.1.2
    4.1.3 https://www.sciencedirect.com/science/article/pii/S0022309399006225#TBL1 

4.2.1  Colorful figure from discomat - Final_MTP presentation + Real table example (from google doc)
4.2.2 by Dhruvil

4.2.3  (Links because it is table + text) + some example in appendix as well

4.3 (kausik) Instead of lot of figures in appendix, can we show only most frequent ones and give references of corner cases

4.4 Kausik

4.4.1 will be removed and a table will be given in the appendix




==> section/2_dup_methodology.tex <==
\section{Methodology}
\label{headings}
In the recent work of Gupta et al. ~\cite{gupta-etal-2023-discomat}, compositions were extracted from MatSci articles, where they distantly annotated the training data and manually annotated the val and test data to find the model's metrics. To identify the challenges for extracting the composition and corresponding processing conditions of the glass along with its properties mentioned under various testing conditions, we have looked into their entire dataset. We used the val and test data from their study, and then randomly selected a satisfactory number of tables or publications as per our requirement and reported our anecdotal findings of the frequency of occurrence of each challenge for composition extraction. Similarly, for property extraction, we used this same val and test dataset and manually annotated the property tables. The annotations were completed by two co-authors, both of them are experienced working in this field and one of them possesses expertise in this discipline. We noted an almost perfect user agreement regarding property identification of around **** and 89.07 for IDs using the Cohen Kappa measure. Disagreements were solved via mutual discussions. We also used their training data and matched the text of tables to the value of the properties stated for that particular publication in the commercial DB INTERGLAD V7.0 ~\cite{interglad}, and distantly identified the property tables in which we also looked for challenges, although all the statistical figures presented in this paper rely on manually annotated data in order to ensure their accuracy.
